Direct Multipath-Based SLAM

In future wireless networks, the availability of information on the position of mobile agents and the propagation environment can enable new services and increase the throughput and robustness of communications. Multipath-based simultaneous localization and mapping (SLAM) aims at estimating the position of agents and reflecting features in the environment by exploiting the relationship between the local geometry and multipath components (MPCs) in received radio signals. Existing multipath-based SLAM methods preprocess received radio signals using a channel estimator. The channel estimator lowers the data rate by extracting a set of dispersion parameters for each MPC. These parameters are then used as measurements for SLAM. Bayesian estimation for multipath-based SLAM is facilitated by the lower data rate. However, due to finite resolution capabilities limited by signal bandwidth, channel estimation is prone to errors and MPC parameters may be extracted incorrectly and lead to a reduced SLAM performance. We propose a multipath-based SLAM approach that directly uses received radio signals as inputs. A new statistical model that can effectively be represented by a factor graph is introduced. The factor graph is the starting point for the development of an efficient belief propagation (BP) method for multipath-based SLAM that avoids data preprocessing by a channel estimator. Numerical results based on synthetic and real data in challenging single-input, single-output (SISO) scenarios demonstrate that the proposed method outperforms conventional methods in terms of localization and mapping accuracy.

==> Figs/scenario/VAconcept.tex <==
\begin{tikzpicture}
%
\def\cx{-0.5}
\def\cy{-2}


%
\def\axone{-1}
\def\ayone{-0.8}


%
\def\px{-3}
\def\py{-2}

%
\def\rot{0}


\tikzset{
anchor0/.pic={ %
\filldraw[draw=white!10!black,fill=black!0,semithick] (0mm,0mm) circle (1mm);
},
anchor1/.pic={ %
\filldraw[draw=black,fill=black!0,semithick,{dash pattern=on 3pt off 1pt}] (0mm,0mm) circle (1mm);
},
anchor2/.pic={ %
\filldraw[draw=white!10!black,fill=black!0,semithick,{dash pattern=on 3pt off 1pt}] (0mm,0mm) circle (1mm);
},
agent/.pic={ %
\filldraw[draw=white!10!black,fill=white!10!black,semithick] (0mm,0mm) circle (0.6mm);
},
zero/.pic={ %
\filldraw[draw=black,fill=black!0,semithick] (0,-0.1) -- (0,0.1) (-0.1,0) -- (0.1,0);
},
mva/.pic={ %
\filldraw[draw=black,fill=black!0,semithick] (-0.75mm,-0.75mm) rectangle (0.75mm,0.75mm);
}
}

\coordinate (coord) at (-4,-2.5); %

\coordinate (p0) at (\px,\py); %
\coordinate (pzero) at (\cx,\cy); %

\coordinate (a1) at (\axone,\ayone);
\coordinate (a2) at ($ (a1) - (0,2*\ayone cm)$);
\coordinate (a3) at ($ (a1) - (2*\axone cm,0)$);

\coordinate (A) at (-4,0); 
\coordinate (B) at (0,0);
\coordinate (C) at (0,-2.66);

\coordinate (wall north one) at (intersection of A--B and a2--p0);
\coordinate (wall east one) at (intersection of B--C and a3--p0);
\coordinate (wall east two) at (intersection of B--C and a1--a3);


%
\draw (p0) pic[rotate=\rot] {agent} node[anchor=south,below left,shift={(0.5mm,0.5mm)}] {\small$\V{p}_{k}$}; 

%
\draw[white!50!black,line width=3pt] (A) -- (B) -- (C);
\draw (A)  node[above=0.5mm] {Surface $1$}; 
\draw (C) node[right=0.5mm] {Surface $2$}; 

%
\draw[blue,line width=0.4mm] (a1) -- (p0) node[pos=0.6,anchor=north,sloped,inner sep=0.5mm] {};
\draw[-,line width=0.3mm,black!10!red] (a1) -- (wall north one) node[pos=0.6,above,sloped,inner sep=0.75mm,anchor=south] {};
\draw[line width=0.2mm,black!10!red] (wall north one) -- (p0); 
\draw[dashed,line width=0.2mm,black!10!red] (wall north one) -- (a2);
\draw[-,line width=0.2mm,black!10!red] (a1) -- (wall east one) node[pos=0.7,sloped,inner sep=0.5mm,anchor=north] {};
\draw[line width=0.2mm,black!10!red] (wall east one) -- (p0);
\draw[dashed,line width=0.2mm,black!10!red] (wall east one) -- (a3);

%
\draw (a1) pic[rotate=0] {anchor0} node[anchor=south west,inner sep=1mm, right=1mm,shift={(-.5mm,3mm)}] {\small$\V{p}^{(1)}_{1}$}; 

%
\foreach \aa in {2,3}
{
  \draw (a\aa) pic {anchor1} node[anchor=north east,inner sep=0.5mm, right=1.5mm] {\small$\V{p}^{(1)}_{\aa}$}; 
}
\draw[dashed,line width=0.2mm,black,shorten <=1mm,shorten >=1mm] (a1) -- (a3);

\begin{pgfonlayer}{back1}
	\tkzMarkRightAngle[draw=black,size=.2,line width=0.2mm](B,wall east two,a3);
	\tkzLabelAngle[dist=-0.15,shift={(0.18mm,-0.3mm)}](B,wall east two,a3){\Large$\cdot$};
\end{pgfonlayer}{back1}

\begin{pgfonlayer}{back1}
	\begin{axis}[
		hide axis,
		at={(coord)}, 
		width = 2cm,
		height =2cm,
		legend to name = legendconcept,
		legend style={legend columns=1,/tikz/every even column/.append style={column sep=0.5cm}, anchor=north,legend cell align=left, fill=none, font=\scriptsize},
		]
		\addlegendimage{white!50!black,line width=3pt}\addlegendentry{Reflecting Surface}
		\addlegendimage{line width=0.4mm, blue}\addlegendentry{LOS Path}
		\addlegendimage{line width=0.2mm, black!10!red}\addlegendentry{Reflected Path}
		\addlegendimage{white!10!black, semithick, mark size=2.5pt, mark=\markA, only marks}\addlegendentry{PA}
		\addlegendimage{color=white!10!black, semithick, draw=none, mark size=2.5pt, mark=\markA, mark options={dash pattern=on 3pt off 1pt, white!10!black}, only marks}\addlegendentry{VA}
		\addlegendimage{white!10!black, semithick, mark size=1.5pt, mark=*, only marks}\addlegendentry{Agent}
		
		\addplot[draw=none] coordinates {(0,0)  (0,0)};
	\end{axis}
\end{pgfonlayer}{back1}

\end{tikzpicture}


==> Figs/scenario/pgfplot.tex <==

%
%
\usetikzlibrary{shapes.misc}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{angles}
\usetikzlibrary{quotes}
\usetikzlibrary{fit}
\usetikzlibrary{graphs}
\usetikzlibrary{patterns}
\usetikzlibrary{petri}
\usetikzlibrary{plotmarks}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{decorations.shapes}
\usetikzlibrary{decorations.text}
\usetikzlibrary{backgrounds}
\usetikzlibrary{calc}
\usetikzlibrary{spy}
\usetikzlibrary{math}

\pgfdeclarelayer{backback1}
\pgfdeclarelayer{back1}
\pgfdeclarelayer{lay1}
\pgfdeclarelayer{backback2}
\pgfdeclarelayer{back2}
\pgfdeclarelayer{lay2}
\pgfdeclarelayer{frontlay}
\pgfsetlayers{backback2,back2,lay2,backback1,back1,lay1,main, frontlay}


\ifthenelse{\equal{\exportFigures}{true}}
{
	\usepgfplotslibrary{external}
	\tikzexternalize[prefix=\tikzfolder,optimize command away=\includepdf]
	\ifthenelse{\equal{\exportFiguresAsPNG}{true}}
	{
		%
		%
		%
		%
		%
		%
		\tikzset
		{   png export/.style={
				external/system call={
					pdflatex \tikzexternalcheckshellescape -halt-on-error --extra-mem-top=10000000 -interaction=batchmode -jobname "\image" "\texsource" && pdftops -eps "\image.pdf" && convert -density 700 -transparent white "\image.pdf" "\image.png"
		}}}
		\tikzset{png export}
		%
		%
	}
	{}
}
{}


%
\newenvironment{customlegend}[1][]{%
    \begingroup
    %
    %
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    %
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%

%
%
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}
\def\addlegendentry{\csname pgfplots@addlegendentry\endcsname}


\newcommand{\pgfref}[1]
{\ifthenelse{\equal{\exportFigures}{true}}
{\tikzexternaldisable\ref{#1}\tikzexternalenable}
{\ref{#1}}}
%
%
%
%

\pgfplotsset{compat=newest} 

\usetikzlibrary{backgrounds}
\tikzstyle{load}   = [ultra thick,-latex]
\tikzstyle{stress} = [-latex]
\tikzstyle{dim}    = [latex-latex]
\tikzstyle{axis}   = [-latex,black!55]


%
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}
\definecolor{darkspringgreen}{rgb}{0.09, 0.45, 0.27}
\definecolor{emerald}{rgb}{0.31, 0.78, 0.47}
\definecolor{forestgreen}{rgb}{0.13, 0.55, 0.13}
\definecolor{green(ryb)}{rgb}{0.4, 0.69, 0.2}
\definecolor{green(pigment)}{rgb}{0.0, 0.65, 0.31}

%
\definecolor{mediumpurple}{rgb}{0.58, 0.44, 0.86}
\definecolor{mediumred-violet}{rgb}{0.73, 0.2, 0.52}

%
\definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73} 

%
\definecolor{mediumcandyapplered}{rgb}{0.89, 0.02, 0.17}

\definecolor{pumpkin}{rgb}{1.0, 0.46, 0.09}

\usetikzlibrary{decorations.pathreplacing,decorations.markings}
\usetikzlibrary{arrows.meta}

\newlength\figureheight 
\newlength\figurewidth 
\usetikzlibrary{patterns,arrows}
\usepgfplotslibrary{colormaps}
\usetikzlibrary{plotmarks}
\pgfplotsset{every axis/.append style={
  label style={font=\normalsize},
  tick label style={font=\scriptsize},
  xticklabel={
   %
   \ifdim \tick pt < 0pt
    %
    \pgfmathparse{abs(\tick)}%
    %
    \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
    %
    \pgfmathprintnumber{\tick}
   \fi}
   }}
\usetikzlibrary{decorations.markings}
\makeatletter
\tikzset{
  nomorepostactions/.code={\let\tikz@postactions=\pgfutil@empty},
  mymarkfixednumber/.style n args={3}{decoration={markings,
    mark= between positions 0.1 and 1 step (1/#3)*\pgfdecoratedpathlength with{%
        \tikzset{#2,every mark}\tikz@options
        %
        \pgfuseplotmark{#1}%
      },  
    },
    postaction={decorate},
    /pgfplots/legend image post style={
        mark=#1,mark options={#2},every path/.append style={nomorepostactions}
    },
  },
}
\tikzset{
  nomorepostactions/.code={\let\tikz@postactions=\pgfutil@empty},
  mymarkfixeddistance/.style n args={3}{decoration={markings,
    mark= between positions 0 and 1 step #3cm with{%
        \tikzset{#2,every mark}\tikz@options
        \pgftransformresetnontranslations%
        \pgfuseplotmark{#1}%
      },  
    },
    postaction={decorate},
    /pgfplots/legend image post style={
        mark=#1,mark options={#2},every path/.append style={nomorepostactions}
    },
  },
}
\tikzset{
  nomorepostactions/.code={\let\tikz@postactions=\pgfutil@empty},
  mymark/.style n args={3}{decoration={markings,
    mark= between positions 0 and 1 step 0.75cm with{%
        \tikzset{#2,every mark}\tikz@options
        \pgftransformresetnontranslations%
        \pgfuseplotmark{#1}%
      },  
    },
    postaction={decorate},
    /pgfplots/legend image post style={
        mark=#1,mark options={#2},every path/.append style={nomorepostactions}
    },
  },
}
\makeatother

%
\definecolor{colA}{rgb}{0,0,1}%
\definecolor{colB}{rgb}{1.00000,0.0,0.00000}%
\definecolor{colC}{rgb}{0,0.7,0}%
\definecolor{colD}{rgb}{0.9,0.0,0.9}%
\definecolor{colE}{rgb}{0,1,1}%
\definecolor{colF}{rgb}{1.00000,0.55,0.00000}%

\def\mylinewidth{0.4}

\def\mymarksize{1.5}
\def\markA{o}
\def\markB{square}
\def\markC{triangle}
\def\markD{diamond}
\def\markE{pentagon}
\def\markF{+}
\pgfdeclareplotmark{markarrow}
{%
  \pgfpathmoveto{\pgfqpoint{\pgfplotmarksize}{0pt}}
  \pgfpathlineto{\pgfqpointpolar{130}{1.5\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpoint{\pgfplotmarksize}{0pt}}
  \pgfpathlineto{\pgfqpointpolar{-130}{1.5\pgfplotmarksize}}
  %
  \pgfusepathqstroke
}




==> LatexInclusion/catechism.tex <==
%----------------------------------------------------------------------------------------%
%                                       C a t e c h i s m                                         %
%----------------------------------------------------------------------------------------%
\section*{Research Paper Catechism\footnote{Adapted from George Heilmeier.}} 

\vspace{0.5cm} 

\be\itemsep3ex

\item What is the big picture? What is the problem and why is it hard?
	\bi
	\item[$\diamond$] The Big Picture: \BigPicture
	\item[$\diamond$] The Problem/Difficulty: \ProblemDifficulty
%	\item[$\diamond$] The Difficulty:
	\ei

\item What are the classical approaches? What is the state-of-the-art and what are the deficiencies?
	\bi
	\item[$\diamond$] Classical Approaches: \ClassicApproach
	\item[$\diamond$] The State-of-the-Art and Deficiencies:  \SOADeficiency
	\item[ ] \mysubsubnote{This is where you make a literature review. Articulate the deficiencies and shortcomings of previous work. Provide references (you can use the first three alphabets of the authors' last names and year, similar to the convention in our database).}
	\ei
	
\item What are the fundamental questions relevant to the problem? How answering to these questions can impact the design, architecture, and operation?
	\bi
	\item[$\circ$] \FundamentalQ
	\item[$\circ$] \EnablingA 
	\item[ ] \mysubsubnote{This is where you persuade the reader that these are fundamental questions, and the answers to these questions will have game-changing impacts.}
	\ei	

\item What are the goals of our paper?
	\bi
	\item[$\diamond$] The Goals:
	\item[ ] \mysubsubnote{Describe the goals at a high level; this should correlate with high-level contributions in Question 6.}
	\ei
		\be
		\item[$\circ$] \Goals 
		\ee		

\item What are we advocating; what is the new technical idea; what is our new view; what is our credence? Why we can succeed now? 
	\bi
	\item[$\diamond$] Advocacy, Idea, View, and Credence:
	\item[ ] \mysubsubnote{For example:}
		\be
		\item[$\circ$] \Advocacy 
		\ee
	\item[$\diamond$] Reasons for Success:
	\item[ ] \mysubsubnote{For example:}
		\be
		\item[$\circ$] \ReasonSuccess 
		\ee
	\ei

\item What are the high-level contributions of our  paper? What are the key contributions of our paper? 
	\bi
	\item[$\diamond$] High-Level Contributions: \HLContribution
	\item[ ] \mysubsubnote{Describe what we do at a high level; this should address the goal that we set out in Question 4; for example:}
		\be
		\item[$\circ$] In this paper, \ldots
		\ee
	\item[$\diamond$] Key Contributions:
	\item[ ] \mysubsubnote{Provide a bulletized list (usually 3-5 bullets, equal number of lines per bullets); for example:}
		\be
		\item[$\circ$] \KeyContribution
		\ee
	\ei


\item Which are the methodologies (analysis, simulation, experimentation, heterogeneous approach) used in this paper? How is the approach verified; how are the results confirmed?
	\bi
	\item[$\diamond$] The Methodologies: Belief propagation, factor graphs, graph neural networks
	\item[$\diamond$] The Verification: The proposed algorithm will be evaluated on nuScenes tracking dataset.
	\ei
	
\item What are the new vision/perspective we provide? What are the lessons learned?
	\bi
	\item[$\diamond$] The New Vision/Perspective: \ConclusiveVision
	\item[$\diamond$] The Lessons Learned/Surprising Results: \ConclusiveLesson
	\ei

\item What is the impact; what are the benefits or merits of the results to a broader community?
	\bi
	\item[$\diamond$] The Impact/Benefit: \Benefit
	\item[ ] \mysubsubnote{Think of strong conclusions for the paper when answering them}
	\ei


\item Where the known results appear in the paper?
	\bi
	\item[$\diamond$] Disclosures: Statistical modeling of the \ac{mot} problem is introduced in Section \ref{sec:model} and the \ac{bp}-based \ac{mot} algorithm is reviewed in \ref{sec:bp}.
	\item[ ] \mysubsubnote{Identify where known results appear in the paper (point to specific section numbers before the paper is written; point to specific section, page, line, equation numbers, etc. after the paper is written).}
	\item[$\diamond$] Sources: \ac{bp}-based \ac{mot} algorithm \cite{WilLau:J14,MeyBraWilHla:J17,MeyKroWilLauHlaBraWin:J18}.
	\item[ ] \mysubsubnote{Identify what are the sources (provide reference, section, page, line, equation numbers, etc. of the sources).}
	\ei

\item What are the key references?
\bi
	\item[ ] \mysubsubnote{List the key references that we used to develop this paper (rather than the references for the state-of-the-art).}
	
	\ac{bp} \cite{KscFreLoe:01,YedFreWei:05,KolFri:B09}; \acp{gnn} \cite{GorMonSca:05, GilSchRilVinDah:17}; \ac{bp} with deep learning \cite{YooLiaXioZhaFetUrtZemPit:19, KucChaTanLuoSonSabErm:20, SatWel:21}; \ac{mot} \cite{BarWilTia:B11, Mah:B07}
% 	object detectors \cite{YinZhoKra:21, ZhuJiaZhoLiYu:19, LanVorCaeZhoYanBei:19}; nuScenes dataset \cite{CaeBanLanVorLioXuKriPanBalBei:20}
	
% 	MOT (``point target''): \cite{BarWilTia:B11,Mah:B07,MeyKroWilLauHlaBraWin:J18}; EOT \cite{HabThaKirGriWak:C11,HamSveSanSor:J12,HabThaThaMalKir:J13
% 	,SchReuWan:C15,CorCar:J18,GenVivBraSolAmi:J15,VivBra:J16,GraOrg:J12,LunGraOrg:J13,BeaReuGraVoVoSch:J16,GraFatSve:J17}: 
\ei

\ee


==> LatexInclusion/defmetric.tex <==
% put your latex definitions here.
% For example: \newcommand{\samplesize}{n}

%---------------------%
% Symbols             %
%---------------------%


%---------------------%
% References        %
%---------------------%
%\newcommand{\fig}[1]{Fig.~\ref{#1}}
%\newcommand{\sect}[1]{Sec.~\ref{#1}}
%\newcommand{\apd}[1]{Appendix~\ref{#1}}
%\newcommand{\eq}[1]{(\ref{#1})}


%--------------------------------------------------------------%
% List: Using description, enumerate, itemize       %
%--------------------------------------------------------------%

\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bl}{\begin{list}}
\newcommand{\el}{\end{list}}
\newcommand{\bt}{\begin{tabbing}}
\newcommand{\et}{\end{tabbing}}

\providecommand{\cbl}{\textcolor{blue}}
\providecommand{\crd}{\textcolor{red}}

%--------------------------------------------------------------%
% Define color specifically for MarkBoth 		  %
%--------------------------------------------------------------%
\definecolor{BLUE}{rgb}{0,0,1}

